Some remarks on modified diagonals

We prove a number of basic vanishing results for modified diagonal classes. We also obtain some sharp results for modified diagonals of curves and abelian varieties, and we prove a conjecture of O'Grady about modified diagonals on double covers.

==> BMmacs <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% First part: fonts
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\catcode`\@=11
\def\hexnumber@#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
        A\or B\or C\or D\or E\or F\fi }
%%
%%  Blackboard bold and msa fonts
%%
\font\tenmsa=msam10  \font\tenmsb=msbm10
\font\eightmsa=msam8 \font\eightmsb=msbm8
\font\sevenmsa=msam7 \font\sevenmsb=msbm7
\font\sixmsa=msam6   \font\sixmsb=msbm6
\font\fivemsa=msam5  \font\fivemsb=msbm5
\newfam\msafam
\textfont\msafam=\tenmsa  \scriptfont\msafam=\sevenmsa
  \scriptscriptfont\msafam=\fivemsa
\edef\msa@{\hexnumber@\msafam}
\newfam\msbfam
\textfont\msbfam=\tenmsb  \scriptfont\msbfam=\sevenmsb
  \scriptscriptfont\msbfam=\fivemsb
\edef\msb@{\hexnumber@\msbfam}
\def\Bbb{\ifmmode\let\next\Bbb@\else
        \def\next{\errmessage{Use \string\Bbb\space only in math 
mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msbfam#1}
%%
%%  \bfit 
%%
\font\tenmib=cmmib10
\font\eightmib=cmmib8
\font\sevenmib=cmmib7
\font\sixmib=cmmib6
\font\fivemib=cmmib5
\newfam\mibfam
\textfont\mibfam=\tenmib  \scriptfont\mibfam=\sevenmib
  \scriptscriptfont\mibfam=\fivemib
\edef\mib@{\hexnumber@\mibfam}
\def\bfit{\ifmmode\let\next\bfit@\else
  \def\next{\errmessage{Use \string\bfit\space only in math mode}}\fi\next}
\def\bfit@#1{\fam\mibfam#1}
%%
%%  \frak (eufm)
%%
\font\teneufm=eufm10
\font\eighteufm=eufm8
\font\seveneufm=eufm7
\font\sixeufm=eufm6
\font\fiveeufm=eufm5
\newfam\eufmfam
\textfont\eufmfam=\teneufm  \scriptfont\eufmfam=\seveneufm
  \scriptscriptfont\eufmfam=\fiveeufm
\edef\eufm@{\hexnumber@\eufmfam}
\def\frak{\ifmmode\let\next\frak@\else
  \def\next{\errmessage{Use \string\frak\space only in math mode}}\fi\next}
\def\frak@#1{\fam\eufmfam#1}
%%
%%  RSFS
%%
\font\teneusm=rsfs10
\font\seveneusm=rsfs7
\font\fiveeusm=rsfs5
\newfam\eusmfam
\textfont\eusmfam=\teneusm  \scriptfont\eusmfam=\seveneusm
  \scriptscriptfont\eusmfam=\fiveeusm
\edef\eusm@{\hexnumber@\eusmfam}
\def\euscr{\ifmmode\let\next\euscr@\else
  \def\next{\errmessage{Use \string\euscr\space only in math mode}}\fi\next}
\def\euscr@#1{\fam\eusmfam#1}
%%
%%      sans serif (sf)
%%
\font\tensf=cmss10
\font\eightsf=cmss8
\font\sevensf=cmss7
\font\sixsf=cmss6
\font\fivesf=cmss5
\newfam\sffam
\textfont\sffam=\tensf  \scriptfont\sffam=\sevensf
  \scriptscriptfont\sffam=\fivesf
\def\hexnumber@#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
        A\or B\or C\or D\or E\or F\fi }
\edef\sf@{\hexnumber@\sffam}
\def\sf{\let\next\sf@\next}
\def\sf@#1{\fam\sffam#1}
%%
%% Special Math chars
%%
\mathchardef\square="0\msa@03
\mathchardef\myleq="3\msa@36
\mathchardef\mygeq="3\msa@3E
\mathchardef\subsetneq="3\msb@28
\mathchardef\exttensor="1\msa@02
\mathchardef\boxplus="0\msa@01
\let\sqtensor=\exttensor
\let\leq=\myleq
\let\geq=\mygeq
\catcode`\@=12

%%
%% Fonts for 8-point
%%
\font\eightrm=cmr8  \font\sixrm=cmr6
\font\eighti=cmmi8  \font\sixi=cmmi6
\font\eightsy=cmsy8 \font\sixsy=cmsy6
\font\eightbf=cmbx8 \font\sixbf=cmbx6
\font\eighttt=cmtt8
\font\eightit=cmti8
\font\eightsl=cmsl8
\font\eighteusm=rsfs7 scaled\magstep1
\font\sixeusm=rsfs5 scaled\magstep1
%%
\catcode`@=11
\newskip\ttglue
\def\eightpoint{\def\rm{\fam0\eightrm}% switch to 8-point type
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti  \scriptfont1=\sixi  \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex   \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \textfont\itfam=\eightit  \def\it{\fam\itfam\eightit}%
  \textfont\slfam=\eightsl  \def\sl{\fam\slfam\eightsl}%
  \textfont\ttfam=\eighttt  \def\tt{\fam\ttfam\eighttt}%
  \textfont\bffam=\eightbf  \scriptfont\bffam=\sixbf
    \scriptscriptfont\bffam=\fivebf  \def\bf{\fam\bffam\eightbf}%
  \textfont\msafam=\eightmsa \scriptfont\msafam=\sixmsa
    \scriptscriptfont\msafam=\fivemsa
  \textfont\msbfam=\eightmsb \scriptfont\msbfam=\sixmsb
    \scriptscriptfont\msbfam=\fivemsb \def\Bbb{\fam\msbfam\eightmsb}%
 \textfont\eusmfam=\eighteusm \scriptfont\eusmfam=\sixeusm
    \scriptscriptfont\eusmfam=\fiveeusm 
 \textfont\eufmfam=\eighteufm \scriptfont\eufmfam=\sixeufm
    \scriptscriptfont\eufmfam=\fiveeufm     
\def\euscr{\fam\eusmfam\eighteusm}%
\def\frak{\fam\eufmfam\eighteufm}%    
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=10pt
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width0pt}%
  \let\sc=\sixrm \let\big=\eightbig \normalbaselines\rm}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}
\catcode`@=12


%%
%% fonts for the title
%%
\font\namefont=cmr12
\font\byfont=cmti12
\font\titlefont=cmbx12


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Second part: layout, sections, counters
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% PAGE SIZE and PAGE LAYOUT:
%%
\hsize16truecm
\vsize23.5truecm
\normalbaselineskip=14.5pt
\normalbaselines

%% Various counters that are used for the chapters, sections etc
%%
\newcount\secno
\def\sectno{\number\secno}
\newcount\ssecno
\def\ssectno{\number\ssecno}
\newcount\referno
\def\refno{\number\referno}
\newcount\equano
\def\equatno{\number\equano}

%% sections
%%
\def\section#1#2{%
\advance\secno by 1\ssecno=0\equano=0\definexref{#2}{\sectno}{section}%
\writenumberedtocentry{section}{#1}{\the\secno}
\vskip2.0\bigskipamount plus 2pt minus 1pt%
\goodbreak\centerline{{\bf \sectno. #1}}\nobreak\ignorespaces}

\def\ssection{\advance\ssecno by 1\equano=0%
\vskip.75\bigskipamount plus 2pt minus 1pt%
\ifnum\ssecno>1\penalty-300\else\nobreak\fi%
\noindent{{\bf \sectno.\ssectno.}}\enspace \ignorespaces}

\def\tocheader{\centerline{{\bf Contents}}%
\vskip.75\bigskipamount plus 2pt minus 1pt}

\def\intro{%
\ssecno=0\equano=0%
\writetocentry{nnsect}{Introduction}
\vskip2.0\bigskipamount plus 2pt minus 1pt%
\goodbreak\centerline{{\bf Introduction}}%
\nobreak\ignorespaces}

\def\ssectionnonr{\equano=0%
\vskip.75\bigskipamount plus 2pt minus 1pt%
\ifnum\ssecno>1\penalty-300\else\nobreak\fi%
\noindent\ignorespaces}

\def\ssectlabel#1{\definexref{#1}{\sectno.\ssectno}{subsection}}

%% used for labels of references:
%%
\def\bibitem#1{\advance\referno by1\definexref{#1}{\refno}{}\item{\hbox to 1.6em{{\rm [\refno]}\hfill}}}

%% macro for numbered equations. 
%%
\def\eqlabel#1{\global\advance\equano by 1%
\leqno{\hbox{\rm (\sectno.\ssectno.\equatno)}}%
\definexref{#1}{\sectno.\ssectno.\equatno}{}}

\def\Romno#1{\uppercase\expandafter{\romannumeral #1}}
\let\romno=\romannumeral

%% macros for the TOC:
%%
\def\leaderfill{\leaders\hbox to.8em{\hss.\hss}\hfill}
\def\tocsectionentry #1#2#3{\line{#2.\quad {\rm #1}\leaderfill\hbox 
to15pt{\hfill #3}}}
\def\tocnnsectentry #1#2{\line{{\rm #1}\leaderfill\hbox to15pt{\hfill #2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Third part: maths
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  Blackboard Bold
%%
\def\mC{{\Bbb C}}
\def\mF{{\Bbb F}}
\def\mG{{\Bbb G}}
\def\mK{{\Bbb K}}
\def\mN{{\Bbb N}}
\def\mP{{\Bbb P}}
\def\mQ{{\Bbb Q}}
\def\mR{{\Bbb R}}
\def\mS{{\Bbb S}}
\def\mU{{\Bbb U}}
\def\mV{{\Bbb V}}
\def\mX{{\Bbb X}}
\def\mZ{{\Bbb Z}}

\def\Ql{\mQ_\ell}

%%  Bold math letters:
%%
\catcode`\@=11
\mathchardef\blambda="0\mib@15
\mathchardef\bmu="0\mib@16
\mathchardef\bnu="0\mib@17
\catcode`\@=12
\def\bi{{\bfit i}}
\def\bj{{\bfit j}}
\def\bJ{{\bfit J}}
\def\bm{{\bfit m}}

%%  Script letters:
%%
\def\cC{{\euscr C}}
\def\cD{{\euscr D}}
\def\cE{{\euscr E}}
\def\cF{{\euscr F}}
\def\cI{{\euscr I}}
\def\cL{{\euscr L}}
\def\cO{{\euscr O}}
\def\cP{{\euscr P}}

%% Fraktur:
%%
\def\gS{{\frak S}}

\def\ga{{\frak a}}
\def\gg{{\frak g}}
\def\gu{{\frak u}}
\def\gz{{\frak z}}

\def\gl{{\frak gl}}
\def\hg{{\frak hg}}
\def\sl{{\frak sl}}
\def\sp{{\frak sp}}

\def\gNS{{\frak g}_\NS}


%%  arrows
%%
\def\stretcharrow{\mathop{\hbox to 15pt{\rightarrowfill}}}
\def\stretchworra{\mathop{\hbox to 15pt{\leftarrowfill}}}
\def\mapright#1{\mathrel{\stretcharrow\limits^{\;\,#1\;\;}}}
\def\mapleft#1{\mathrel{\stretchworra\limits^{\;\;#1\;\,}}}
\def\mapdown#1{\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapup#1{\Big\uparrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\let\maprighto=\mapright
\def\maprightu#1{\mathrel{\stretcharrow\limits_{\;\,#1\;\;}}}
\def\mapdownr#1{\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapdownl#1{\llap{$\vcenter{\hbox{$\scriptstyle#1$}}$}\Big\downarrow}
\def\mapdownlr#1#2{\llap{$\vcenter{\hbox{$\scriptstyle#1$}}$}\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#2$}}$}}
\def\sizedmapright#1#2{\setbox0=\hbox{$\mapright{#1}$}%
\mathrel{\mathop{\hbox to \wd0{\rightarrowfill}}\limits^{\;\,#2\;\;}}}

\def\isomarrow{\mapright{\sim}}
\def\twoheadrightarrow{\rightarrow\kern -8pt\rightarrow}
\let\tto=\longrightarrow
\def\jjoinrel{\mathrel{\mkern-3.3mu}}
\def\hooklongrightarrow{\lhook\jjoinrel\longrightarrow}
\let\longhookrightarrow=\hooklongrightarrow


%%  "operator names"
%%
\def\A{{\rm A}}
\def\AJ{{\rm AJ}}
\def\Alb{{\rm Alb}}
\def\CH{{\rm CH}}
\def\Corr{{\rm Corr}}
%\def\DB{{\rm DB}}
\def\End{{\rm End}}
\def\Fil{{\rm Fil}}
\def\Gal{{\rm Gal}}
\def\GL{{\rm GL}}
\def\Hom{{\rm Hom}}
\def\Inn{{\rm Inn}}
\def\Irrep{{\rm Irrep}}
\def\Ker{{\rm Ker}}
\def\Lef{{\rm Lef}}
\def\Nrd{{\rm Nrd}}
\def\NS{{\rm NS}}
\def\Pic{{\rm Pic}}
\def\Rep{{\rm Rep}}
\def\Res{{\rm Res}}
\def\SL{{\rm SL}}
\def\Sp{{\rm Sp}}
\def\Spec{{\rm Spec}}
\def\Stab{{\rm Stab}}
\def\Standard{{\rm St}}
\def\Sym{{\rm Sym}}

\def\alb{{\rm alb}}
\def\adm{{\rm adm}}
\def\alg{{\rm alg}}
\def\char{{\rm char}}
\def\cont{{\rm cont}}
\def\depth{{\rm depth}}
\def\der{{\rm der}}
\def\fd{{\rm fd}}
\def\gon{{\rm gonality}}
\def\hom{{\rm hom}}
\def\id{{\rm id}}
\def\incl{{\rm incl}}
\def\lfss{{\rm lfss}}
\def\mult{{\rm mult}}
\def\num{{\rm num}}
\def\opp{{\rm op}}
\def\pol{{\rm pol}}
\def\pr{{\rm pr}}
\def\prim{{\rm prim}}
\def\pt{{\rm pt}}
\def\red{{\rm red}}
\def\sep{{\rm sep}}
\def\sub{{\rm sub}}
\def\sym{{\rm sym}}
\def\top{{\rm top}}
\def\trace{{\rm tr}}
\def\trans{{\rm trans}}
\def\transpose{{\rm t}}

%% some categories:
%%
\def\Mod{{\sf Mod}}
\def\Mot{{\sf Mot}}
\def\SmProj{{\sf SmProj}}
\def\Var{{\sf V}}
\def\Vect{{\sf Vect}}

%% various other things:
%%
\let\ol=\overline 
\let\ul=\underline

\let\tempcolon=\colon
\def\colon{\tempcolon\,}

\def\transp{{}^\transpose}
\let\core=\boxplus
\def\age#1{{[#1]}}

\def\smalldot{{\raise.25ex\hbox{${\scriptscriptstyle \bullet}$}}}

%%
%% the next one is a little special: we want \sim to be used for an
%% 'adequate equivalence relation' but it often appears as an ordinary
%% symbol (as opposed to a relation). So we define a special macro '\aer'
%% for this:
%%
\mathchardef\aer="0218


\def\Proof{\noindent{\it Proof.\/}\enspace}
\def\Pf#1{\noindent{\it #1.\/}\enspace}
\def\QED{\unskip\nobreak\hfill\hbox{$\mskip 9mu minus 5mu \square$}}

\def\kbar{{\bar{k}}}
\def\Kbar{{\bar{K}}}
\def\Ktilde{{\tilde{K}}}
\def\Qbar{{\ol{\mQ}}}
%\def\Af{\mA_\fin}

\def\chargp{\mX}
\def\Four{\cF}
\def\unitmot{{\bf 1}}
\def\UEA{\mU}


\def\Romno#1{\uppercase\expandafter{\romannumeral #1}}
\let\romno=\romannumeral

\def\boxit#1{\leavevmode\hbox{\vrule\vtop{\vbox{\hrule\kern2pt\hbox{\vphantom{X}\thinspace#1\thinspace}}\kern2pt\hrule}\vrule}}

%% macros for time:
%%
\newcount\minuten
\newcount\uren
\newcount\temp
\minuten=\the\time
\uren=\the\time
\divide\uren by 60
\temp=\uren
\multiply\temp by -60
\advance\minuten by \the\temp
\def\tijd{\ifnum\minuten<10 \the\uren:0\the\minuten\else \the\uren:\the\minuten\fi}
%%
%% END OF MACRO FILE
%%
